T-TAMER: Provably Taming Trade-offs in ML Serving

As machine learning models continue to grow in size and complexity, efficient serving faces increasingly broad trade-offs spanning accuracy, latency, resource usage, and other objectives. Multi-model serving further complicates these trade-offs; for example, in cascaded models, each early-exit decision balances latency reduction against potential accuracy loss. Despite the pervasiveness and importance of such trade-offs, current strategies remain largely heuristic and case-specific, limiting both their theoretical guarantees and general applicability. We present a general framework, T-Tamer, which formalizes this setting as a multi-stage decision process, where the objective is to determine both when to exit and which model to consult. Our main result shows that recall (i.e., the ability to revisit earlier models) is both necessary and sufficient for achieving provable performance guarantees. In particular, we prove that strategies without recall cannot obtain any constant-factor approximation to the optimal trade-off, whereas recall-based strategies provably attain the optimal trade-off in polynomial time. We validate our analysis through experiments on synthetic datasets and early-exit workloads for vision and NLP benchmarks. The results show that recall-based strategies consistently yield efficient accuracy-latency trade-offs. We hope this work provides a principled foundation for bridging heuristic practice with theoretical guarantees in the design of early-exit and cascaded models.

==> content/fix_transition.tex <==
\subsection{Static Transition for Multiple Lines}\label{subsec:1_hyperbox_rapid_mix}

We now study the case where the precedence graph consists of multiple lines. In the case of static cost, the equivalent reward table can be computed more efficiently using the following theorem.

\begin{theorem}[Markov Chain with Static Cost]\label{thm:MC_constant_cost}
Under Ass.~\ref{ass:MC_cost}, the reward of each line follows an (infinite) Markov chain (Def.~\ref{def:app:MC}), and each probe incurs a constant cost $c$. For any $i \in [k-1]$, $p_{i,k}>0$, we assume that the equivalent reward $ \phi $ depends only on $ y $ as the current maximum reward and $ x $ as the current reward. The optimal strategy is to continue if $ \phi(y, x) > y $ and stop if $ \phi(y, x) \leq y $.

\end{theorem}
In this case, the equivalent reward $ \phi $ is \textit{independent} of the current box index. Thus, the equation derived from \textit{Bellman’s principle of optimality} corresponds to a \textit{fixed-point iteration} where the variables are $ \phi $ under different states. We show that this iteration leads to a \textit{unique solution} and converges rapidly. For details, see Appendix~\ref{subsec:app:rapid_mix_MC_static_cost}.

\begin{lemma}[Rapid Convergence of Max Reward]\label{lem:dist_max_reward}
Given any directed line subgraph $\hyperb := \{b_1,\ldots, b_n\}$ of the precedence graph with transition matrix $P_M$, assume that $P_M$ is irreducible and aperiodic. There exists a stable distribution $\pi$ such that given $\delta \in (0,1)$, with probability $1- \delta$, \\ for $t \geq \max \{ 2 \frac{C_{\trans}}{ (\sum_{i = j}^{k} \pi_i) (1 - \alpha_{\trans})},  \frac{\log (1 / \delta)}{\log (1 - (\sum_{i = j}^{k} \pi_i) / 2)} \}$ 
\begin{align*}
    \Pr [R_{\max}(t) \geq v_j] \geq 1- \delta
\end{align*} 
for any $j \in [k]$, where we define the max reward of the first $t$ boxes in $\hyperb$ as  $R_{\max} (t) := \max \{R_1,\ldots, R_t\}$.
\end{lemma}

\begin{proof}

From Lem.~\ref{lem:app:convege_line_stable}, given any subset $S \subseteq V = \{v_1,\ldots, v_k\}$, we have for $\pi_S := \sum_{v \in S} \pi_v$:
\begin{align*}
  \pi_S - C_{\trans} \alpha^t_{\trans} \leq \Pr [R_t \in S] \leq \pi_S + C_{\trans} \alpha^t_{\trans}. 
\end{align*}

Next, we lower bound the probability that $R_{\max} (t) = v_k$, where we define $\pi_{\min} = \min_{j \in [k]} \pi_j$, $\eps_t := \min \{ \pi_{\min},  C_{\trans} \alpha^t_{\trans} \}$, and $\bar{\eps}_t := \frac{1}{t} \sum_{t_0 \in [t]} \eps_{t_0}$, as
% then when $t \to \infty$, the minimum of this definition would be $C_{\trans} \alpha^t_{\trans}$.
\begin{align*}
    &\Pr (R_{\max} (t) = v_k) = 1 - \Pi_{t_0 \in [t]} \Pr[R_t < v_k] \geq \\
 & 1 - \Pi_{t_0 \in [t]} (1 - \pi_k + \eps_{t_0}) \geq 1 - (1 - \pi_k)^t (1 +\frac{ \bar{\eps}_t} { 1 - \pi_k})^t,
\end{align*}
where the first equality follows by definition, the second follows by the convergence to stable distribution, and the third follows from AM-GM (Lem.~\ref{lem:app:AM_GM}).

Next, we upper bound $\bar{\eps}_t$:
\begin{align*}
    & \bar{\eps}_t =  \frac{1}{t} \sum_{t_0 \in [t]} \eps_{t_0} 
    \leq  \frac{1}{t} \sum_{t_0 =1}^{\infty} C_{\trans} \alpha_{\trans}^{t_0} \
    =  \frac{1}{t} C_{\trans} \frac{1}{1 - \alpha_{\trans}}.
\end{align*}
Thus, $\Pr[R_{\max} (t) = v_k] \geq 1 - [1 - \pi_k + \frac{1}{t} \frac{C_{\trans}}{(1 - \alpha_{\trans})}]^t$.

Notice that for $t \geq 2 \frac{C_{\trans}}{ \pi_k (1 - \alpha_{\trans})}$, we have:
\begin{align*}
    (1 - \pi_k + \frac{1}{t} \frac{C_{\trans}}{1 - \alpha_{\trans}}) \leq 1 - \pi_k / 2.
\end{align*}
Given $\delta>0$, for $t \geq \max \{ 2 \frac{C_{\trans}}{ \pi_k (1 - \alpha_{\trans})}, \frac{ \log (1 / \delta)}{\log (1 - \pi_k / 2)} \}$,  
\begin{align*}
    & \Pr[R_{\max} (t) = v_k] \geq 1 - (1 - \pi_k + \frac{1}{t} \frac{C_{\trans}}{1 - \alpha_{\trans}})^t \\
    & \geq 1 - (1 - \pi_k/2)^t \geq 1 - \delta.
\end{align*}

\noindent Following the same logic, we could lower bound the probability that $R_{\max} \geq v_j$.
% i.e.,  given $\delta > 0$, for $t \geq \max \{ 2 \frac{C_{\trans}}{ (\sum_{i = j}^{k} \pi_i) (1 - \alpha_{\trans})}, \log (1 / \delta) / \log (1 - (\sum_{i = j}^{k} \pi_i) / 2) \}$, $\Pr [R_{\max} \geq v_j] \geq 1- \delta$. 
\end{proof}

The lemma implies that when the precedence graph is a directed line, there exists a near-optimal policy that explores at most $\tilde{\Theta}(1)$ boxes. This result directly leads to the following theorem. For more details, refer to Appendix~\ref{subsec:app:multi_line_general}.



\begin{theorem}[Near Optimal Probing, Single Line]\label{thm:greedy_optimal_single_line}
Given a Markovian Pandora’s box with static transition, where the precedence graph is a single-line $ \hyperb $ and the transition matrix $ \trans $ is irreducible, aperiodic, and associated with a stable distribution $ \pi $, there exists a constant $C_{\trans}>0$ and $\alpha_{\trans} \in (0,1)$, that, given any $\delta \in (0,1)$, lets  $t_{\delta} = \max \{ 2 \frac{C_{\trans}}{ \pi_k (1 - \alpha_{\trans})},  \frac{\log (1 / \delta)}{\log (1 - \pi_k / 2)} \}$. Then, the expected utility from optimal probing on the subgraph $ \hyperb|t_{\delta} $, containing only the first $ t_{\delta} $ boxes of $ \hyperb $, is near optimal, i.e.,
\begin{align*}
   \OPT (\hyperb|{t_\delta}) \geq   \OPT(\hyperb) - 2\delta v_k,
\end{align*}
where $\OPT(\hyperb)$ is the expected utility from optimal probing graph $\hyperb$.
\end{theorem}


This theorem implies that it is near optimal to truncate any hyperbox by its first $t_\delta$ steps, which we generalize to the multi-line setting. More details are in Appendix~\ref{subsec:app:multi_line_general}.

\begin{theorem}[Near Optimal Probing, Multi Lines]\label{thm:greedy_optimal_multi_line}
Given a Markovian Pandora’s box with static transition, where the precedence graph $G$ consists of $q$ directed lines $ \hyperb_1, \ldots, \hyperb_q$, suppose every transition matrix $P_j$ of each $\hyperb_j, j \in [q]$ is irreducible, aperiodic, and associated with a stable distribution $ \pi(j) $. There exists constant $C>0$ and $\alpha \in (0,1)$, that, given any $\delta \in (0,1)$, let $t_{\delta} = \max \{ 2 \frac{C}{ \pi^* (1 - \alpha)},  \frac{\log (1 / \delta)}{\log (1 - \pi^* / 2)} \}$, where $\pi^* = \max_{j \in [q]} \pi (j)_k$. Then, the expected utility from optimal probing on the subgraph $ \cup_{j \in [q]} (\hyperb_j |t_{\delta}) $, containing only the first $ t_{\delta} $ boxes of each hyperbox, is near optimal, i.e.,
\begin{align*}
   \OPT [\cup_{j \in [q]} (\hyperb_j |t_{\delta})] \geq   \OPT(G) - 2q\delta v_k,
\end{align*}
where $\OPT(G)$ is the expected utility from optimal probing graph $G$. 
\end{theorem}




% \yy{Merge this lemma with previous lemma on the single hyperbox. }
% \begin{lemma}[Properties of Equivalent Reward, Single Line]\label{lem:property_one_line}
% Given a hyperbox $\hyperb := \{b_1, \ldots, b_m\}$, 

% \squishlist
%     \item The Equivalent Reward could be solved by the following Bellman's equation:
%     \begin{align*}
%         \phi(X,v_0,t) = \max \{ X, -c_t +  \sum_{v \in V} \Pr [R^t = v | R^{t-1} = v_0] \phi (\max\{ x, R^{t} \}, v, t+1)  \}
%     \end{align*}
%     \item If the reward and cost follows a Markov chain with time dependent cost  with transition matrix $P \in \R^{k \times k}$ (Ass.~\ref{ass:MC_cost}), this simplifies to:
%     \begin{align*}
%         \phi(X,v_i,t) = \max \{ X, -c_t +  \sum_{ j \in [k]} p_{ij} \phi (\max\{ X, v_j \}, v_j, t+1)  \}
%     \end{align*}
%     \item The generalized reservation value is the smallest $X$ satisfies $\phi(X, v_i,t ) = X$. 
%     \item Given any $t$, the Equivalent Reward $\phi(X, v,t )$ is within $2 \delta v_k $ of the $\phi_{t + t_\delta}(X, v,t)$, i.e., 

%     \begin{align*}
%         \phi(X, v,t ) \leq \phi_{t + t_\delta}(X, v,t) + 2 \delta v_k 
%     \end{align*}
%      where $t_{\delta} = \max \{ 2 \frac{C_{\trans}}{ (\sum_{i = j}^{k} \pi_i) (1 - \alpha_{\trans})},  \frac{\log (1 / \delta)}{\log (1 - (\sum_{i = j}^{k} \pi_i) / 2)} \} $, and $\phi_{t + t_\delta}$ denote the Equivalent Reward on the subhyperbox $\hyperb|_{t + t_\delta}$.
% \squishend
% \end{lemma}


% \begin{proof}
% We begin by showing each of the arguments sequentially. 
% \squishlist
%     \item Notice that if a stopping time is optimal for box $t \to \infty$, then this stopping time is also optimal for box $t+1 \to \infty$, given any realization of the $t$-th box. Hence, we denote $\tau$ as the optimal stoping time, then we have:
%     \begin{align*}
%         \phi(X, v_0, t) &= \max \{ X,  \E[\max_{t_0 = t}^{\tau} R^{t_0} - \sum_{t_0 = t}^{\tau} c_{t_0} ]\} \\
%         & = \max \{ X, -c_{t} + \E[ \max \{ \max \{R^{t}, X \}, \max_{t_0 = t+1}^{\tau} R^{t_0} - \sum_{t_0 = t+1}^{\tau} c_{t_0} \} ] \} \\
%         & = \max \{ X, -c_t +  \sum_{v \in V} \Pr [R^t = v | R^{t-1} = v_0] \phi (\max\{ X, R^{t} \}, v, t+1)  \}
%     \end{align*}
%     where the first line follows from the definition of $\phi$, the second line follows from separating the term for the t-th box, the third line follows from opening up the expectation term.

%     \item Following the above notations, writing $\Pr [R^t = v_j | R^{t-1} = v_i]$ as $p_{i,j}$ for every $i,j \in [k]$ gives us the desired result. 

%     \item This follows from the optimality of $X$. \yy{maybe we need to elaborate this. }
%     \item This proof performs similarly as the one in Thm.~\ref{thm:greedy_optimal}.  WLOG, we denote the optimal stopping for $\hyperb$ as $\tau^*$, and the optimal stopping for $\hyperb|_{t+t_\delta}$ as $\tau_{t+t_\delta}$. We construct a stopping time $\bar{\tau}$ such that $\bar{\tau} = \tau^*$ for $\tau^* \leq t_\delta + t$, and $\bar{\tau} = t_\delta$ for $\tau^* > t_\delta + t$. Following the notations in Def.~\ref{def:stat_dist}, we have:

%     \begin{align*}
%         & \Pr( \tau^* \leq t + t_\delta) \E[\phi(X, v,t)|\tau^* \leq t_\delta+t] \\
%         = & \phi(X, v,t) - \Pr( \tau^* > t_\delta + t) \E[\phi(X, v,t)|\tau^* > t_\delta+t] \\
%         \geq & \phi(X, v,t) - \delta v_k 
%     \end{align*}
%     %where the first equality follows from the law of total expectation, the second inequality follows from Lem.~\ref{lem:dist_max_reward}.

%     Next, notice that for scenarios that $\tau^* > t_\delta + t$, $\bar{\tau}^*$ would stop at the last box when probing $\hyperb| t+t_{\delta}$, we have: 
%     \begin{align*}
%         \E[\phi_{t + t_\delta}(X, v,t) ] \geq & \E[\phi^{\bar{\tau}}_{t + t_\delta}(X, v,t) ] \\
%         \geq & \phi(X, v,t) - \delta v_k  + \E[\phi^{\bar{\tau}}_{t + t_\delta}(X, v,t)|\tau^* > t_\delta+t] \Pr [\tau^* > t_\delta+t] \\
%         \geq &  \phi(X, v,t)- \delta v_k - \delta v_k
%      \end{align*}
%     where the first inequality is due to the (sub)optimality of $\bar{\tau}$ on $\hyperb | t_{\delta} + t$, and the second inequality follows from the Lem.~\ref{lem:dist_max_reward} that $\Pr[\tau^* \leq t_\delta + t] \geq \Pr[R_{\max} (t_\delta) = v_k)] \geq 1-\delta$. Regarding the last inequality, notice that if $\Pr[\tau^* > t_\delta + t] >0$, it's necessary that $v_k - \sum_{t \in [t_\delta]} c_t >0$, otherwise $\tau^*$ is not optimal. Thus, $ \E[\phi^{\bar{\tau}}_{t + t_\delta}(X, v,t)|\tau^* > t_\delta+t] \geq - \sum_{t \in [t+t_\delta]} c_t \geq - v_k $.



% \squishend    
% \end{proof}

% The last point indicates that the generalized reservation value by the truncation also fluctuates only by a small amount, hence we can use lookahead strategy to compute the GR within a small range. 





==> content/fix_transition_forest.tex <==
\newpage
\subsection{Extension to Forest}\label{subsec:transition_forest}

We now show that for the forest setting, there still exists an induced subgraph with a much smaller size that guarantees roughly $1/2$-approximation of the expected payoff. We first define the \textit{approximate ratio}.

\begin{definition}[Approximate Ratio]\label{def:approx_ratio}
    A strategy $\pi$ is said to be a $C$-approximation of the Markovian Pandora's box  if, given any strategy $\hat{\pi}$, the expected utility of $\pi$ satisfies
    \begin{align*}
        \E [\max_{i \in \mathcal{O}(\pi)} R_i - \sum_{i \in \mathcal{O}(\pi)} c_i] \geq C \cdot  \E[\max_{i \in \mathcal{O}(\hat{\pi})} R_i] - \sum_{i \in \mathcal{O}(\hat{\pi})} c_i],
    \end{align*}
    where $\mathcal{O}(\pi)$ denotes the random set selected by strategy $\pi$. 
\end{definition}

We next present a lemma stating that there exists a non-adaptive strategy that guarantees the utility of the best adaptive strategy.\footnote{As proven in Thm.3~\cite{bfll20}, this originally holds for order constraints with independent boxes, and their proof generalizes easily to our setting with a forest precedence graph.}

\begin{lemma}[Adaptivity Gap~\cite{bfll20}]\label{lem:forest_adaptivity}
    Consider the Markovian Pandora's box with a forest precedence graph. Then, for every adaptive strategy $\hat{\pi}$, there exists a non-adaptive strategy $\pi$ that obtains $1/2$ approximation. 
\end{lemma}

We can now present our results on a (rougly) $1/2$ approximation for the forest setting. 

% the c can be retrieved via depth first search. 
\begin{theorem}[$1/2$ Approximation, Forest]\label{thm:forest_approx}

Given a Markovian Pandora’s box with static transition, where the precedence graph $G$ is a forest precedence graph, for any $\delta \in (0,1)$, there exists an algorithm that finds a best fixed-line subgraph $\hyperb$ within $\Delta(G)^{\tilde{\Theta}(1)}$ time, such that given any alternative adaptive policy $\pi$, 
    \begin{align*}
        \E [\max_{i \in \mathcal{O}(\pi)} R_i - &\sum_{i \in \mathcal{O}(\pi)} c_i] \geq \\
        &1/2 \cdot  \E[\max_{i \in \mathcal{O}(\hat{\pi})} R_i] - \sum_{i \in \mathcal{O}(\hat{\pi})} c_i] -q \delta,
    \end{align*}
where $\Delta(G)$ is the degree and $q$ is the number of trees in $G$. 
    
\end{theorem}



==> content/fix_transition_multibox.tex <==
\subsection{Extension To Multiple Hyperboxes}\label{subsec:transition_multi_line}

In this section, we show that for a given $\delta$, selecting a $\delta$-dependent induced subgraph ensures that optimal probing within the subgraph still yields a near-optimal expected payoff.

\yy{Maybe truncating to a sufficient small tree and enumerate over all the possible combinations? Now it's computationally efficient. = =. }
\begin{theorem}
    
\end{theorem}

\begin{proof}
\squishlist
    \item Lower bound the probability that for all the hyperbox, $\max_t R_t = v_k $ appeared.
    \item Optimality of Probing by optimal stopping according to GRV. 
    \item End. 
\squishend
\end{proof}
\yy{This is for the most general setting}

\yy{say something like, our proof follows same intuition of the proof in the original Weitzman's paper. }

\yy{write some clarification like, what policies could be treated as pandora's box with random reward and random cost, actually, for any fully adaptive or partially adaptive strategy, we can model this. }




\iffalse

\begin{lemma}[Weitzman's Rule under Independence]\label{lem:GPR_id_optimal}
    Given a collection of $n$ independent Markovian hyperboxes, it's optimal to probe the hyperboxes in the decreasing order of their generalized reservation value, condition on any competitive reward $X$.  
\end{lemma}

\begin{proof}
   \yy{Actually we need to show this lemma by similar intuitions as in Ruimin's proof for the multiple independent boxes w/ no return...} 
\end{proof}

In this lemma, we aim at using the value function of the hyperbox to show the optimality of the ordering. 

\begin{lemma}[Weitzman's Rule under Markovian Dependency]\label{lem:GPR_markov_optimal}
Given three hyperboxes $A, B, C$ with the following property:
\squishlist
    \item The payoff of $B$ (hence the value function) is independent of $A$ and $C$.
    \item The payoff of $C$ depends on $A$ in a Markovian fashion, i.e., for any possible value $x$ of $\util(C)$. 
    \begin{align*}
        \Pr[\util(C) = x | \util(A), \util(B) ] = \Pr [\util(C) = x | \util(A) ]
    \end{align*}
    \item The generalized reservation value $\sigma (A) > \sigma(C)$, given any realizations of $A$\footnote{Notice that here $\sigma(A)$ is not a random variable, but $\sigma(C)$ is a random variable depends on $A$. }, i.e., for any possible value of $x$ of $A$: 
    \begin{align*}
        \sigma (A) \geq [\sigma(C) | A = x]
    \end{align*}
    \item We have a precedence constraint that $A$ must be probed before $C$. 
\squishend
Suppose we can optimal stop inside the hyperboxes, and we cannot return once we switch to other hyperboxes, conditioned on any competitive reward $X$, the optimal probing strategy is to probe these boxes in decreasing order of their generalized reservation value. 
\end{lemma}

\yy{see if we can show this conclusion for $C$ can be both dependent on $A$ and $B$.}

\begin{proof}
    \squishlist
        \item $\sigma (B) > \sigma (A)$: 
        
        \begin{itemize}
            \item First we treat $A \to C$ as a single hyperbox, i.e., $D$, then by lemma???, the generalized reservation value of $D$ is smaller than $\sigma (B)$. Then by lemma.~\ref{lem:GPR_markov_optimal}, the optimal order of forcing $AC$ together is $B \to A \to C$.
            \item Next, we consider orderings that $A$ is not neighboring $C$ in the ordering. There is only one $A \to B \to C$. 
            \item It remains to show that optimal probing according to $B \to A \to C$ have higher expected payoff than optimal probing according to $A \to B \to C$.
        \end{itemize}
        \item $\sigma (A) \geq \sigma (B)$.
        \begin{itemize}
            \item When $A$ neighboring $C$, the optimal order is $A \to C \to B$, according to similar reasoning above. 
            \item When $A$ is not neighboring $C$, there is only one order $ A \to B \to C$.
            \item Notice that for both order, $A$ must be probed first, after that the payoff distribution of $C$ is fixed and independent of hyperbox $B$, hence we are able to use Lem.~\ref{lem:GPR_id_optimal} to rank $B$ and $C$. Hence, the optimal ranking is to rank $A, B, C$ according to their generalized reservation value. 
        \end{itemize}
        
    \squishend
\end{proof}

\fi

==> content/forest.tex <==
\section{Exact Optimization for Forest}\label{sec:forest}
We now describe how to use previous solutions from the multi-line setting to derive a optimal fully adaptive strategy (i.e., probing according to GRV) for tree and forest structures. We first define a \textit{minimal tree}. 

\begin{definition}[Tree, Branch Vertex, Minimal Tree]\label{def:tree}
A directed \emph{tree} $\T$ is a connected DAG where removing any edge disconnects the graph. A directed \emph{forest} is a DAG whose components are trees. A \emph{branch} vertex in a directed tree is a vertex with at least $2$ outgoing edges. A \emph{minimal tree} is a tree whose strict subgraphs contain no branch vertices.
\end{definition}

The key intuition behind our algorithm is that probing the root $r$ in a minimal tree reduces the induced graph $\bar{G}$ to \textit{multiple lines}, enabling us to apply our solutions in Section~\ref{sec:multi_boxes}. By extending Lem.~\ref{lem:equ_box}, we contract $\bar{G}$ into a single box with random cost $\hat{b}$ and use the following to calculate the equivalent reward for $r$ given the current reward $x$:
  \begin{align*}
     \Phi(x,r) = & \max\{x, \E[\max\{R_r, x\} - c_r], \\
     & \quad \E[\max\{R_r, x, R_{\hat{b}}\} - c_r - c_{\hat{b}}]\}.
 \end{align*}
The terms in the max operator correspond to the utility of not opening $r$, opening only $r$, and opening $r$, respectively, while optimally exploring the remaining nodes. The GRV is fully specified once $\phi$ is known.


Next, we present our algorithm for computing the GRV for every box, which iteratively finds and contracts the minimal trees of the underlying graph into a line, thus eliminating all branch vertices iteratively.\footnote{In the presence of opened boxes, for any unopened box $i$, we apply the algorithm to the subtree rooted at $i$ to compute its GRV.}


\begin{algorithm}[!ht]\caption{Updating GRV, Forest}\label{alg:pd_forest}
\begin{algorithmic}[1]
    \Require An instance of a Markovian Pandora's box with precedence graph $G$ as a forest. 
    % The precedence graph $G$, the cost of each boxes, the reward distribution of all $q$ root vertices $\mathcal{R} = \{r_1, r_2, \ldots, r_q\}$, and the probability transition matrix of each directed edge $P_{i,j}$, for box $i$ and box $j$.  
    \State $\hat{G} \gets G$, $t \gets 1$.
    \While {there are minimal trees in graph $G_0$.}
    \For {every minimal tree $\T_i$ with root $r_i$.}
        \For {every possible state $R_{r_{i}}$ of $r_i$. }
        \State Condition on $R_{r_{i}}$, compute $\phi$ and GRV $\sigma$ for every possible state for vertices/boxes in $\T_i \setminus \{r_i\}$.
        \State Contract $\T_i \setminus \{r_i\}$ into one vertex $\hat{v}_i$, compute its reward and cost distribution condition on $R_{r_{i}}$. 
        \EndFor
        \State Update $\hat{G}$ accordingly. 
    \EndFor 
    \EndWhile
    \State Compute the GRV of remaining boxes.
\end{algorithmic} 
\end{algorithm}

See App.~\ref{sec:app:omit_forest} for more details regarding the optimality and polynomial runtime of probing according to the GRV.

% Since each contraction step is optimal, the strategy probes the box with the highest GRV and stops when the current max reward exceeds the highest available GRV. Proof of correctness and polynomial runtime is in App.~\ref{sec:app:omit_forest}.




==> content/ind_growth.tex <==
\subsection{Independent Growth in Model Capability}

\yy{story: gradient descent}

\begin{assumption}[Independent Growth in Model Capability]\label{assu:ind_growth}
 For each box $i \in [n]$, let the model capability be $\theta_i$. The incremental model capability is defined as $\delta_i = \theta_i - \theta_{i-1}$, where $\delta_i$ follows a distribution $\Delta_i$, and $\E[\delta]_i >0 $. For any $i \neq j \in [n]$, $\Delta_i$ and $\Delta_j$ are independent. The reward of box $i$ is:
    \begin{align*}
        R_i = f\left(\sum_{j \in [i]} \delta_j\right) = f(\theta_i),
    \end{align*}
    where $f: \mathbb{R} \to \mathbb{R}$ is a concave function, capturing diminishing returns as cumulative capability increases.
    
\end{assumption}

\subsubsection{Full Information Setting}\label{subsec:full_info}

\begin{lemma}[Full Information: Independent Growth]\label{lem:full_info_independent}
The optimal strategy for setting in Ass.~\ref{assu:ind_growth} is that, given current time $i$ and capability $\theta_i$, to search over all $j$, if there exist any $j$ such that $\E[f(\theta_j)] - \sum_{l \in [j]} c_l >0$. 
\yy{the difficulty lies in that $ f(\E[\theta_j]) >  \E[f(\theta_j)]$ for concave function. }

    
\end{lemma}

\yy{this setting seems less interesting =.= since the solution is trivial in some sense...}


==> content/multi_line.tex <==
\section{Exact Optimization for Multiple-Line Constraints}\label{sec:multi_boxes}
% \hf{Might be helpful to draw some figures to illustrate different settings we consider. A figure with a line, multiple lines, and forests. } \yy{Added in the intro.}

In this section, we introduce the notion of time-adaptive generalized reservation value (t-GRV) for multi-line settings and show that the optimal strategy is to probe the available box with the highest current t-GRV. The main technique is to reduce the problem of modeling probing across different lines to probing a sequence of (random) single equivalent boxes with correlated costs. Here, “random” refers to the random start and end indices defining the range of each equivalent box. We begin by introducing the definition of a box with cost correlated with reward. 

\yy{put definition of t-GRV of the multi-line setting here. }


\yy{please check whether all the content use the word ``correlated" instead of the ``random" cost. }

\begin{definition}[Box with Correlated Cost]\label{def:pandora_box_random_cost}
A box $b$ is classified as an \textit{equivalent box with random cost} if it has a hidden reward $R$ and an opening cost $c$, where both $R$ and $c$ are \textit{random variables} drawn from \textit{known} distributions $\mathcal{D}_R$ and $\mathcal{D}_c$, respectively. Here, the opening cost $c$ varies and is \textit{correlated} with the reward $R$; we denote the joint distribution of $\mathcal{D}_R$ and $\mathcal{D}_c$ as $\Gamma$. 
\end{definition}

Next, we show how a hyperbox can be equivalently represented by a single box, such that both the reward distribution and the t-GRV are preserved. This equivalent representation plays a key role in our proof: Given a hyperbox and any stopping time, we model the distribution of the resulting payoff to that of an equivalent box. Since the rewards of all boxes share the same support, the payoff’s support lies in a space of dimension at most $k \times n$, where $n$ and $k$ are the number of boxes and the number of distinct support values, respectively. See Appendix~\ref{sec:app:multi_line} for more details. 

\yy{draw a graph here to explain the separation of graphs.}


\begin{lemma}[Equivalent Box for Hyperbox]\label{lem:equ_box}
For a stopping time $\tau$ and a hyperbox $\hyperb := \{b_1, \ldots, b_n\}$, there exists a box $\hat{b}$ with random cost (Def.~\ref{def:pandora_box_random_cost}) such that following $\tau$ over $\hyperb$ has the same utility distribution as $\hat{b}$.
\end{lemma}
% \hf{I agree with this, but I think the support of this equivalent single box maybe exponentially large? I need to understand proof a bit more. } \yy{add more details in the paragraph above this lemma. }



% \subsection{Algorithm for Multiple Lines}\label{subsec:alg_multi_line}

% \yy{define filteration. }
% \begin{algorithm}[!ht]
% \caption{Markov Pandora's Box, Multi Lines}
% \label{alg:generalize_weitz_multi}
% \begin{algorithmic}[1]
% \State {\bf Input:} Miniboxes $B$, ordering constraints encoded as $L_1, \ldots, L_k$.   
% \State Initialize $t \gets 0$, $\Vmax \gets 0$, $j \gets 1$, $\F_t \gets \O$
% \State Initialize the feasible minibox set $L$. 
% \While{$\Vmax \leq \max_{p \in L} \sigma_p | \F_t$} 

%     \Comment{If the max value seen so far is less than all the Weitzman's thresholds of the candidates, the algorithm proceeds. }
%     \State $i_t \gets \max_{p \in L} \sigma_p | \F_t$. \Comment{Pick the minibox with max threshold.}
%     \State Probe the box $i_t$, observe $M_{i_t}$.
%     \State $\F_{t+1} \gets \F_{t} \cup \{ \M_{i_t}  = M_{i_t} \}$. \Comment{Update the Information. }
%     \If{$M_t > \Vmax$}
%     \State $j \gets t$, $\Vmax \gets M_t$. \Comment{Update the maximum value. }
%     \EndIf
%     \State Find the first available box $m_t$ after $i_t$, $L \gets L \setminus {i_t} \cup {m_t}$. \Comment{Update the candidate set.}
    
%     \State Calculate $\sigma_{m_t} | \F_{t+1}$ \Comment{Estimate the Weitzman's threshold of the next box, based on current information.  } % In the multi-path setting, this update is sufficient. 
%     \If{$\sigma_{m_t} | \F_{t+1} < \Vmax$.}
%     \State {\bf Return} $j$ and $\Vmax$.
%     \Else{}
%     \State $t \gets  t+1$. \Comment{Continue in the loop.}
%     \EndIf
% \EndWhile
% \State {\bf Return} $j$ and $\Vmax$.
% \end{algorithmic}
% \end{algorithm}

We begin by presenting a key lemma for our main theorem, which establishes that under certain Markovian correlations, the t-GRV remains an optimal decision rule. 


\begin{lemma}[Probing Equivalent Boxes]\label{lem:three_box_lemma}
Given the three Pandora's boxes $A, B, C$ with random cost (Def.~\ref{def:pandora_box_random_cost}) \textit{and} the following properties:
\squishlist
    \item The reward and cost of $B$ are independent of the reward and cost of $A$;
    \item The reward and cost (hence payoff) of $C$ depend on both $A$ and $B$ in a Markovian fashion;
    \item The reservation value $\sigma (A) > \sigma (B)> \sigma(C)$ given any realizations of $A$ and $B$\footnote{Here, $\sigma(C)$ is a random variable that depends on $A$ and $B$.}, i.e., for any possible value of $x$ of $A$ and possible value of $y$ of $B$, is 
    \begin{align*}
        \sigma (A) \geq \sigma (B) \geq [\sigma(C) | R_{A} = x, R_{B} = y];
    \end{align*}

    \item A precedence constraint that $A$ and $B$ must be probed before $C$; 
\squishend
then, conditioned on any current best reward $X$, 
%\hf{what does competitive reward mean?}\yy{fixed.}
the optimal probing strategy is $A \prec B \prec C$. 
\end{lemma}
We show this lemma by first principles, where we compare the utility of the ordering $A \prec B \prec C$ with that of $B \prec A \prec C$ through a case-by-case analysis on the outcomes from the joint distribution of $A$, $B$, and $C$ and aggregate them by the law of total expectation. For more details on the complete proof, see Appendix.~\ref{sec:app:multi_line}. 

Now we are ready to establish the optimality of t-GRV for the multi-line setting, showing that probing the available boxes based on their latest t-GRV maximizes the expected payoff. 

\begin{theorem}[Optimality of t-GRV for Multi-Line Markovian Pandora's Box]\label{thm:ML_MPB}
Given a Markovian Pandora’s box instance whose precedence graph consists of $m$ lines, the optimal strategy for maximizing expected utility is to probe the hyperboxes based on their latest t-GRV. \yy{add reference here. }
\end{theorem}
\vspace{-5mm}

% \hf{I remember we considered two different models -- can return back to the same Hyperbox, or cannot come back once leaving the hyperbox. Which model is this? Also, I think at some point we have a nice proof using Gittin's index -- what is that for?  } \yy{We can return back to the same hyperbox; Gittin's index is for both the single line setting, and the multi-line setting w/ no return. }

% %interchange arguments
% \begin{proof}
%  We denote $n^*$ as the hyperbox with the highest GRV when no boxes are opened, and we denote $\sigma^0_{n^*}$ as the value of this GRV. We denote $n \neq n^*$ as another fixed hyperbox. WLOG, we denote the GRV of the hyperbox as the GRV of the first unopened box conditioned on the realized reward. Let $\pi^*$ denote the fully adaptive strategy that at every iteration, probe the hyperbox with the highest current GRV. We use $U(\pi)$ to denote the expected utility of probing (and hence optimal stopping) according to (adaptive) ordering $\pi$.


% We first restricted ourselves to (adaptive) strategies that once enters the hyperbox, will only leave the hyperbox if the competitive unopened but available GRV is higher: We consider a collection of (adaptive) strategies/ordering of the boxes $\pi^{(0)}, \pi^{(1)}, \ldots, \pi^{(q)}$ that converges to the optimal (adaptive) ordering. We first describe the base policy $\pi^{(0)}$:  $\pi^{(0)}$ starts by first probing the hyperbox $n$, then probing the hyperboxes according to $\pi^*$. Inductively, the strategy $\pi^{(q)}$ is obtained via first probing the box $n^*$ until the next box in line has an updated GRV smaller than $\sigma_{n^*}^0$, then probing the box according to $\pi^{(q-1)}$. Thus, when $q \rightarrow \infty$, we get that the policy converges to our proposed optimal ordering $\pi$. 

% We defer the proof of $U(\pi^{(1)}) \leq U(\pi^{(0)})$ to Lem.~\ref{lem:base_case_GRV} in App.~\ref{sec:app:multi_line}. The key intuition is that both strategies follow the same order (roughly) after both strategy entered $2$ hyperboxes. Consequently, the remaining boxes in this agreed order can be treated as a single box with a random cost, dependent on the preceding two hyperboxes Markovianly. This structure allows us to apply Lem.~\ref{lem:three_box_lemma} for comparison.

% Next, we show that for any $q$, $U (\pi^{(q-1)}) \leq U (\pi^{(q)})$. Since $\pi^{(q)}$ and $\pi^*$ agree on the selection of the first $q-1$ hyperboxes, they are identical while exploring these hyperboxes. \textit{WLOG}, we compare their utilities \textit{conditioned on} both strategies continuing until they enter the $q$-th hyperbox. In $\pi^{(q-1)}$, the $q$-th hyperbox is $n$, whereas in $\pi^{(q)}$, it is the one with the highest current GRV, denoted as $\hat{n}^q$. By the optimality of $\hat{n}^q$ and applying Lemma~\ref{lem:base_case_GRV}, we conclude that the expected payoff of $\pi^{(q-1)}$ is strictly less than that of $\pi^{(q)}$.
% \end{proof}


\begin{proof}
We denote $n^*$ as the hyperbox with the highest GRV when no boxes are opened, and we denote $\sigma^0_{n^*}$ as the value of this GRV. We denote $n \neq n^*$ as another fixed hyperbox. WLOG, we denote the GRV of the hyperbox as the GRV of the first unopened box conditioned on the realized reward. Let $\pi^*$ denote the fully adaptive strategy that probes the hyperbox with the highest current GRV. 
%We want to show that there is no strategy that could outperform $\pi^{*}$ by induction on the number of boxes. 
% We use $U(\pi)$ to denote the expected utility of probing (and hence optimal stopping) according to (adaptive) ordering $\pi$.

We now show that no strategy can outperform $\pi^{*}$ by induction on the number of boxes. 

\textbf{Base Case}. Given only two boxes, it is immediately clear that $\pi^*$ is the optimal strategy.

\textbf{Induction Step}. Assume $\pi^*$ is optimal for $q-1$ boxes; we show that it remains optimal for $q$ boxes. If the optimal strategy starts by probing the hyperbox $n^*$, then by induction, $\pi^*$ is already optimal for $q$ boxes.
%\jm{I don't see this. I see $\pi^*$ is defined to open the hyperbox with highest GRV, but I don't see why (a) this choice is optimal, or (b) why the remainder of the problem reduces to the $q-1$ box case (are these boxes hyperboxes or actual boxes? if actual boxes, then I suppose I see since opening a box means one fewer box. But I don't know if $q$ refers to the total number of boxes or the number of available boxes.}


Now, suppose the best strategy $\hat{\pi}$ starts with a hyperbox $n$ whose GRV $\sigma_n^{0}$ is lower than $\sigma_{n^*}^{0}$. By the induction hypothesis, $\hat{\pi}$ follows $\pi^*$ after probing its first hyperbox. The order of $\hat{\pi}$ is as follows: probe $n$ until the next box’s GRV falls below $\sigma_{n^*}^{0}$, then switch to $n^*$, and finally proceed optimally through the remaining boxes.

We construct a new strategy $\bar{\pi}$ with strictly higher expected utility, contradicting the optimality of $\hat{\pi}$. The order of $\bar{\pi}$ is: probe $n^*$ first, then switch to $n$ when the next box’s GRV falls below $\sigma_{n^*}^{0}$, and finally continue optimally as in $\hat{\pi}$. 

Notice that the GRV for the segments containing $n^*$ is $\sigma_{n^*}^{0}$, but the GRV for the segments containing $n$ is smaller than $\sigma_n^{0}$, and that both strategies explore the same segments of $n^*$ and $n$ but in different orders. We can apply Lemma~\ref{lem:three_box_lemma} to show that $\bar{\pi}$ yields a higher expected payoff than $\hat{\pi}$. This leads to a contradiction. Thus, by induction, we show that $\pi^*$ remains optimal for any number of boxes.
\end{proof}
%\vspace{-5mm}
Finally, we present the theorem showing that GRV can be implemented in polynomial time and space. Given the optimality of the GRV under the optimal policy, each box's GRV depends only on the realized rewards within its hyperbox, enabling the payoff table to compute GRVs of all states \emph{without} iterative updates to the adaptive order. See Appendix.~\ref{sec:app:multi_line} for further details.

\begin{theorem}[Generalized Reservation Value, Multi Lines]\label{thm:GMR_path}
The GRV for a multi-line setting can be implemented in polynomial time and space. 
\end{theorem}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

